Dynamics-based halo model for large scale structure

Accurate modelling of the one-to-two halo transition has long been difficult to achieve. We demonstrate that physically motivated halo definitions that respect the bimodal phase-space distribution of dark matter particles near halos resolves this difficulty. Specifically, the two phase-space components are overlapping and correspond to: 1) particles \it orbiting \rm the halo; and 2) particles \it infalling \rm into the halo for the first time. Motivated by this decomposition, Garc\'ia [R. Garc\'ia et. al., MNRAS 521, 2464 (2023)] advocated for defining haloes as the collection of particles orbiting their self-generated potential. This definition identifies the traditional one-halo term of the halo--mass correlation function with the distribution of orbiting particles around a halo, while the two-halo term governs the distribution of infalling particles. We use dark matter simulations to demonstrate that the distribution of orbiting particles is finite and can be characterised by a single physical scale $r_{\rm h}$, which we refer to as the \it halo radius. \rm The two-halo term is described using a simple yet accurate empirical model based on the Zel'dovich correlation function. We further demonstrate that the halo radius imprints itself on the distribution of infalling particles at small scales. Our final model for the halo--mass correlation function is accurate at the $\approx 2\%$ level for $r \in [0.1,50]\ h^{-1}\ Mpc$. The Fourier transform of our best fit model describes the halo--mass power spectrum with comparable accuracy for $k\in [0.06, 6.0]\ h\ Mpc^{-1}$.

==> authorlist.tex <==
\author[Salazar et al.]{Edgar Salazar$^{1}$\thanks{E-mail: edgarmsc@arizona.edu}, Eduardo Rozo$^{1}$, Rafael Garc\'ia$^{1}$, Nickolas Kokron$^{4,5}$, Susmita Adhikari$^2$, \and Benedikt Diemer$^{3}$, Calvin Osinga$^{3}$
\\
$^{1}$Department of Physics, University of Arizona, Tucson, AZ 85721, USA \\
$^{2}$Department of Physics, Indian Institute of Science Education and Research, Homi Bhaba Road, Pashan, Pune 411008, India\\
$^{3}$Department of Astronomy, University of Maryland, College Park, MD 20742, USA\\
$^{4}$Department of Astrophysical Sciences, Princeton University, Princeton, NJ, 08540, USA\\
$^{5}$School of Natural Sciences, Institute for Advanced Study, Princeton, NJ, 08540, USA\\
% $^{4}$Centre for Astrophysics and Planetary Science, Racah Institute of Physics, The Hebrew University, Jerusalem 91904, Israel\\
% $^{5}$Department of Physics, Yale University, New Haven, CT 06520, USA
}

